Unveiling the Magic of Code Reasoning through Hypothesis Decomposition and Amendment

The reasoning abilities are one of the most enigmatic and captivating aspects of large language models (LLMs). Numerous studies are dedicated to exploring and expanding the boundaries of this reasoning capability. However, tasks that embody both reasoning and recall characteristics are often overlooked. In this paper, we introduce such a novel task, code reasoning, to provide a new perspective for the reasoning abilities of LLMs. We summarize three meta-benchmarks based on established forms of logical reasoning, and instantiate these into eight specific benchmark tasks. Our testing on these benchmarks reveals that LLMs continue to struggle with identifying satisfactory reasoning pathways. Additionally, we present a new pathway exploration pipeline inspired by human intricate problem-solving methods. This Reflective Hypothesis Decomposition and Amendment (RHDA) pipeline consists of the following iterative steps: (1) Proposing potential hypotheses based on observations and decomposing them; (2) Utilizing tools to validate hypotheses and reflection outcomes; (3) Revising hypothesis in light of observations. Our approach effectively mitigates logical chain collapses arising from forgetting or hallucination issues in multi-step reasoning, resulting in performance gains of up to $3\times$. Finally, we expanded this pipeline by applying it to simulate complex household tasks in real-world scenarios, specifically in VirtualHome, enhancing the handling of failure cases. We release our code and all of results at https://github.com/TnTWoW/code_reasoning.

==> arc_detailed_prompt.tex <==



\begin{table*}[ht!]
    \caption{Comparison between LM-induced rules on MiniARC with and without task-specific heuristics. We show examples where heuristics are helpful (top) and not helpful (bottom) for rule induction. \texttt{0} maps to \texttt{black}.}
    \vspace{-2mm}
    \centering
    \scalebox{0.8}{
    \begin{tabular}{ccc}
    \toprule
    \textbf{Examples} & \textbf{w/o Heuristics} &  \textbf{w/ Heuristics} \\
    \midrule
    \thead{\includegraphics[width=0.3\linewidth]{figures/arc_example_good.pdf}}  & \thead{For each row in the input array, the \\ corresponding output row is generated by \\ taking the first element from the  current row, \\ the second element from the first row,  the \\ third element from the current row,  the fourth \\ element from the second row and the fifth \\ element from the first row. If  the first element \\ of the current row is 0, then the entire output \\ row becomes 0.} & \thead{The input grid is mirrored along its main \\ diagonal, i.e., the diagonal from the top-left \\  corner to the bottom-right corner. The color  \\ mapping remains the same.} \\
    \midrule
    \thead{\includegraphics[width=0.3\linewidth]{figures/arc_example_bad.pdf}}  & \thead{For a given 5x5 matrix, copy the first two \\ values of the first row to the third and fourth \\ positions of the fourth row and the first two  \\ values of the second row to the third and \\ fourth positions of the third row. Then, copy \\ the second value of the second row to the last \\ position of the last row. Leave all the other \\ positions unchanged.} & \thead{The output grid is formed by taking the existing \\ colored cells (non-zero numbers) from the top-\\left corner of the input grid, and creating a \\ mirror image of this pattern  in the bottom-right \\ corner. This mirror image involves not only \\ flipping the pattern along the central vertical and \\ horizontal axes, but also rotating the position of \\ the colors one position to the right in each cell. \\ The rest of the cells remain black (0).} \\
    \bottomrule
    \end{tabular}
    }
    \label{tab:example_heuristics}
\end{table*}

